Revisiting the Complexity of and Algorithms for the Graph Traversal Edit Distance and Its Variants

The graph traversal edit distance (GTED), introduced by Ebrahimpour Boroojeny et al.~(2018), is an elegant distance measure defined as the minimum edit distance between strings reconstructed from Eulerian trails in two edge-labeled graphs. GTED can be used to infer evolutionary relationships between species by comparing de Bruijn graphs directly without the computationally costly and error-prone process of genome assembly. Ebrahimpour Boroojeny et al.~(2018) propose two ILP formulations for GTED and claim that GTED is polynomially solvable because the linear programming relaxation of one of the ILPs always yields optimal integer solutions. The claim that GTED is polynomially solvable is contradictory to the complexity results of existing string-to-graph matching problems. We resolve this conflict in complexity results by proving that GTED is NP-complete and showing that the ILPs proposed by Ebrahimpour Boroojeny et al. do not solve GTED but instead solve for a lower bound of GTED and are not solvable in polynomial time. In addition, we provide the first two, correct ILP formulations of GTED and evaluate their empirical efficiency. These results provide solid algorithmic foundations for comparing genome graphs and point to the direction of heuristics. The source code to reproduce experimental results is available at https://github.com/Kingsford-Group/gtednewilp/.

==> all_tri_proof.tex <==
\begin{lem}
    There exist two unidirectional, edge-labeled Eulerian graphs $G_1$ and $G_2$ such that $\GTED(G_1, G_2)$ is not equal to the optimal solution of ILP version of~\boundarylp where the boundary matrix is defined by $T^{all}(G_1,G_2)$ instead of $T(G_1,G_2)$.
\end{lem}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/alltri.png}
    \caption{(a) An example of two edge labeled Eulerian graphs $G_1$ (top) and $G_2$ (bottom). (b)~The alignment graph $\alngraph(G_1,G_2)$. The cycle with red edges is the path corresponding to $\GTED(G_1, G_2)$. Red solid edges are matches with cost 0 and red dashed-line edge is mismatch with cost 1.}
    \label{fig:alltri}
\end{figure}

\begin{proof}
    Let two Eulerian graphs $G_1$ and $G_2$ be three-node cycle graphs with labels \texttt{A,T,G} and \texttt{A,T,C} on each edge~(Figure~\ref{fig:alltri}(a)). Suppose we assign costs to alignment graphs following Levenshtein edit distance. It is obvious that $\GTED(G_1, G_2) = 1$, and a path in $\alngraph(G_1, G_2)$ that has the same cost has three diagonal edges as shown in Figure~\ref{fig:alltri}(b). We denote this solution $x_{gted}$ where $x_e = 1$ for edges on the path and $x_e = 0$ otherwise. It is easy to see that $x_{gted}$ is a feasible solution to ILP version of~\boundarylp with boundary matrix defined by $T^{all}(G_1,G_2)$.
    %Note that this is a feasible solution to \emph{AG Boundary ILP} with boundary matrix defined by $\Tr^{all}$ as shown in the proof of Theorem~\ref{thm:lpequal}.
    
    However, $x_{gted}$ is not the optimal solution to this modified ILP.  From $x_{gted}$, we can perform an additional boundary operation using the triangle $[(u_0,v_0),(u_1,v_1),(u_2,v_2)]$, which is a triangle in $T^{all}(G_1,G_2)$ but not in $T(G_1,G_2)$:
    \begin{align*}
        x_{new} &=x_{gted}+\partial[(u_0,v_0),(u_1,v_1),(u_2,v_2)]\times (-1) \\
        &=[(u_0,v_0),(u_1,v_1)]+[(u_1,v_1),(u_2,v_2)] \\
        &~~~+[(u_2,v_2),(u_0,v_0)] \\
        &~~~-\partial[(u_0,v_0),(u_1,v_1),(u_2,v_2)] \\
        &=[(u_0,v_0),(u_1,v_1)]+[(u_1,v_1),(u_2,v_2)] \\
        &~~~+[(u_2,v_2),(u_0,v_0)] - [(u_0,v_0),(u_1,v_1)] \\
        &~~~-[(u_1,v_1),(u_2,v_2)]-[(u_2,v_2),(u_0,v_0)] \\
        &=0.
    \end{align*}
    $x_{new}$ is a zero vector yields an objective value $0$ of the modified ILP, which apparently is different from $\GTED(G_1, G_2)$.
\end{proof}
The choice of triangles to construct the boundary matrix in~\boundarylp is not trivial and cannot be arbitrary. While our definition of $T(G_1,G_2)$ may not be the only valid one that results in Theorem~\ref{thm:lpequal}, other alternatives are not within the scope of our discussion. 

==> figures/alngraph_bowtie_c3.tex <==
\begin{center}
\begin{tikzpicture}[
every node/.style={circle,draw,inner sep=0pt,minimum size=3mm,node font=\tiny},
r/.style={red},
]
\foreach[count=\bi] \b in {a,b,c,d,e} {
	\foreach[count=\ci] \c in {a,b,c} {
		\node at (\bi,-\ci) (\b\c) {$\b\c$};
	}
};
\draw[->] (aa) edge (ab)
(aa) edge[r] (ba)
(aa) edge[r] (bb)
(ab) edge (ac)
(ab) edge (bb)
(ab) edge (bc)
(ac) edge[r,bend left] (aa)
(ac) edge[r] (ba)
(ac) edge[r] (bc)
(ba) edge[r] (bb)
(ba) edge[r] (ca)
(ba) edge (cb)
(bb) edge[r] (bc)
(bb) edge (cb)
(bb) edge (cc)
(bc) edge[r,bend right] (ba)
(bc) edge[r] (ca)
(bc) edge[r] (cc)
(ca) edge[bend right] (aa)
(ca) edge (ab)
(ca) edge (cb)
(ca) edge (da)
(ca) edge (db)
(cb) edge[bend left] (ab)
(cb) edge (ac)
(cb) edge (cc)
(cb) edge (db)
(cb) edge (dc)
(cc) edge[r,bend left] (aa)
(cc) edge[r,bend left] (ac)
(cc) edge[r,bend right] (ca)
(cc) edge (da)
(cc) edge (dc)
(da) edge (db)
(da) edge (ea)
(da) edge (eb)
(db) edge (dc)
(db) edge (eb)
(db) edge (ec)
(dc) edge[bend right] (da)
(dc) edge (ea)
(dc) edge (ec)
(ea) edge[bend right] (ca)
(ea) edge (cb)
(ea) edge (eb)
(eb) edge[bend left] (cb)
(eb) edge (cc)
(eb) edge (ec)
(ec) edge[bend left] (ca)
(ec) edge[bend left] (cc)
(ec) edge[bend right] (ea);
\end{tikzpicture}
\end{center}

==> figures/bowtie.tex <==
\begin{tikzpicture}[baseline=(a.north),
every node/.style={circle,draw,inner sep=0pt,minimum size=2.5mm,node font=\tiny}
]
\node at (0,-0.25) (a) {$a$};
\node at (0, 0.25) (b) {$b$};
\node at (0.5,0) (c) {$c$};
\node at (1,-0.25) (d) {$d$};
\node at (1,0.25) (e) {$e$};

\draw[->] (a) edge (b) 
		  (b) edge (c) 
		  (c) edge (a) 
		  (c) edge (d) 
		  (d) edge (e) 
		  (e) edge (c);
\end{tikzpicture}

==> figures/c3.tex <==
\begin{tikzpicture}[baseline=(c.north),
every node/.style={circle,draw,inner sep=0pt,minimum size=2.5mm,node font=\tiny},
]
\node at (0,0) (a) {$a$};
\node at (0.5,0.25) (b) {$b$};
\node at (0.5,-0.25) (c) {$c$};

\draw[->] (a) edge (b)
		  (b) edge (c)
		  (c) edge (a);
\end{tikzpicture}

==> figures/mobius_bowtie_c3.tex <==
\begin{center}
\begin{tikzpicture}[every node/.style={circle,draw,inner sep=0pt,minimum size=3mm,node font=\tiny},]
\node[red] at (0,0) (bc) {$bc$};
\node at (1,0) (bb) {$bb$};
\node at (2,0) (aa) {$aa$};
\node[green] at (0,-1) (ca) {$ca$};
\node at (1,-1) (ba) {$ba$};
\node at (2,-1) (ac) {$ac$};
\node at (3,-1) (cc) {$cc$};
\node[red] at (3,-2) (bc2) {$bc$};
\node[green] at (4,-2) (ca2) {$ca$}; 

\draw (bc) edge (bb)
           edge (ca)
           edge (ba)
      (bb) edge (ba)
           edge (aa)
      (aa) edge (ba)
           edge (ac)
           edge (cc)
      (ca) edge (ba)
      (ba) edge (ac)
      (ac) edge (cc)
           edge (bc2)
      (cc) edge (bc2)
           edge (ca2)
      (bc2) edge (ca2);
\end{tikzpicture}
\end{center}

==> gted_np_proof.tex <==
\begin{thm}\label{thm:gtednp}
\GTED is NP-complete.
\end{thm}
\begin{proof}
We reduce from the \textsc{Hamiltonian Path} problem, which asks whether a directed, simple graph $G$ contains a path that visits every vertex exactly once. Here simple means no self-loops or parallel edges. Let $\langle G=(V,E)\rangle$ be an instance of \textsc{Hamiltonian Path}, with $n=|V|$ vertices. The reduction is almost identical to that presented in~\citet{eulerw}, and from here until noted later in the proof the argument is identical except for the technicalities introduced to force unidirectionality (and another minor change described later). The first step is to construct the Eulerian closure of  $G$, which is defined as $G'=(V',E')$ where
\begin{equation}
V' = \{v^{in}, v^{out} : v \in V\} \cup \{w\},
\end{equation}
and $E'$ is the union of the following sets of edges and their labels:
\begin{itemize}
\item $E_1 = \{(v^{in},  v^{out}) : v \in V\}$,  labeled \texttt{a},
\item $E_2 = \{(u^{out}, v^{in}) : (u,v) \in E\}$,  labeled \texttt{b},
\item $E_3 = \{(v^{out}, v^{in}) : v \in V\}$, labeled \texttt{c},
\item $E_4 = \{(v^{in}, u^{out}) : (u,v) \in E\}$, labeled \texttt{c},
\item $E_5 = \{(u^{in},w) : u \in V\}$, labeled \texttt{c},
\item $E_6 = \{(w,u^{in}) : u \in V\}$, labeled \texttt{b}.
\end{itemize}
Since $G'$ is connected and every outgoing edge in $G'$ has a corresponding antiparallel incoming edge, $G'$ is Eulerian. It is not unidirectional, so we further create $G''$ from $G'$ by adding dummy nodes to each pair of antiparallel edges and labelling the length-2 paths so created with \texttt{x\#}, where \texttt{x} is the original label of the split edge (\texttt{a}, \texttt{b}, or \texttt{c}) and \texttt{\#} is some new symbol (shared between all the new edges). We call these length-2 paths introduced to achieve unidirectionality ``split edges''.

We now argue that $G$ has a Hamiltonian path iff $G''$ has an Eulerian trail that spells out 
\begin{equation}
q = \texttt{a\#}(\texttt{b\#a\#})^{n-1}(\texttt{c\#})^{2n-1}(\texttt{c\#b\#})^{|E| + 1}.
\end{equation}
If such an Eulerian trail exists, then the trail starts with spelling the string $\texttt{a\#}(\texttt{b\#a\#})^{n-1}$, which corresponds to a Hamiltonian trail in $G$ since it visits exactly $n$ ``vertex split edges'' (type $E_1$, labeled \texttt{a\#}) and each vertex split edge can be used only once (since it is an Eulerian trail). Further, successively visited vertices must be connected by an edge in $G$ since those are the only \texttt{b\#} split edges in $G''$ (except those leaving $w$, but $w$ must not be involved in spelling out $\texttt{a\#}(\texttt{b\#a\#})^{n-1}$, since entering $w$ requires using a split edge labeled $\texttt{c\#}$).

\newcommand\pred{\text{pred}}

For the other direction,  if a $G$ has a Hamiltonian path $v_1,\dots,v_n$, then walking that sequence of vertices in $G''$ will spell out $\texttt{a\#}(\texttt{b\#a\#})^{n-1}$. This path will cover all $E_1$ edges and the $E_2$ edges that are on the Hamiltonian path. Retracing the path so far in reverse will use $2n-1$ split edges labeled \texttt{c\#}, consuming the $(\texttt{c\#})^{2n-1}$ term in $q$ and covering all nodes' reverse vertex edges $E_3$ (since the path is Hamiltonian). The reverse path also covers the $E_4$ edges corresponding to reverse Hamiltonian path edges. Our Eulerian trail is now ``at'' node $v_1^{in}$.

What remains is to complete the Eulerian walk covering (a)~edges and their antiparallel counterparts corresponding to 
edges in $G$ that were not used in the Hamiltonian path, and (b)~the edges adjacent to node $w$. To do this, define $
\pred(v)$ be the vertices $u$ in $G$ for which edge $(u,v)$ exists \emph{and} $u$ is not the predecessor of $v$ along 
the Hamiltonian path. For each $u\in\pred(v_1)$, traverse the split 
edge labeled \texttt{c\#} to $u^{out}$ then traverse the forward split edge labeled $\texttt{b\#}$ back to $v_1^{in}$. This results in a string 
$(\texttt{c\#b\#})^{|\pred(v_1)|}$. Once the predecessors of $v_1$ are exhausted, traverse the split edge labeled \texttt{c\#} from $v_1^{in}$
into node $w$ and then traverse the split edge labeled \texttt{b\#} to $v_2^{in}$. This again generates a \texttt{c\#b\#} string. Repeat the process, covering the edges of 
$v_2$'s predecessors and returning to $w$ to move to the next node along the Hamiltonian path for each node 
$v_3,\dots,v_n$. After covering the predecessors of $v_n^{in}$, go to $v_1^{in}$ through the remaining edges in $E_5$ and $E_6$, $(v_n^{in},w)$ and $(w, v_1^{in})$, which 
completes the Eulerian tour. This covers all the edges of $G''$. The word spelled out in this last section of the Eulerian trail is a sequence of repetitions of \texttt{c\#b\#}, with one repetition for 
each  edge that is not in the Hamiltonian path ($|E|-n+1$) and all of the edges in $E_5$ and $E_6$ for entering and leaving each node ($2n$), with a total of $|E|+1$ repetitions, which is the final $(\texttt{c\#b\#})^{|E| + 1}$ term in $q$.

This ends the slight modification of the proof in~\citet{eulerw}, where the differences are (a)~the introduction of the \texttt{\#} characters and (b)~using the exponent $|E|+1$ of the final part of $q$ instead of $|E|+n+1$ as in~\citet{eulerw} since we create $w$-edges only to $v^{in}$ vertices. (This second change has no material effect on the proof, but reduces the length of the string that must be matched.)

Now, given an instance $\langle G=(V,E)\rangle$ of \textsc{Hamiltonian Path}, with $n=|V|$ vertices, we construct 
$G''$ as above (obtaining a unidirectional Eulerian graph) and create a DAG $C$ spelling out $q$. Note that 
$|\Sigma|=4$ and $G''$ and $C$ can be constructed in polynomial time. $\GTED(G'',C)= 0$ if and only if an Eulerian path in $G''$ spells out $q$, since there can be no indels or mismatches. By the above argument, an 
Eulerian tour that spells out $q$ exists if and only if $G$ has a Hamiltonian path.
\end{proof}

